Teaching Code LLMs to Use Autocompletion Tools in Repository-Level Code Generation

Code large language models (LLMs) face limitations in repository-level code generation due to their lack of awareness of repository-level dependencies (e.g., user-defined attributes), resulting in dependency errors such as undefined-variable and no-member errors. In this work, we introduce ToolGen, an approach that integrates autocompletion tools into the code LLM generation process to address these dependencies. ToolGen comprises two main phases: Trigger Insertion and Model Fine-tuning (Offline), and Tool-integrated Code Generation (Online). During the offline phase, ToolGen augments functions within a given code corpus with a special mark token, indicating positions to trigger autocompletion tools. These augmented functions, along with their corresponding docstrings, are then used to fine-tune a selected code LLM. In the online phase, ToolGen iteratively generates functions by predicting tokens step-by-step using the fine-tuned LLM. Whenever a mark token is encountered, ToolGen invokes the autocompletion tool to suggest code completions and selects the most appropriate one. We conduct comprehensive experiments to evaluate ToolGen's effectiveness in repository-level code generation. To facilitate this evaluation, we create a benchmark comprising 671 real-world code repositories and introduce two new dependency-based metrics: Dependency Coverage and Static Validity Rate. The results demonstrate that ToolGen significantly improves Dependency Coverage by 31.4% to 39.1% and Static Validity Rate by 44.9% to 57.7% across the three LLMs, while maintaining competitive or improved performance in widely recognized similarity metrics such as BLEU-4, CodeBLEU, Edit Similarity, and Exact Match. On the CoderEval dataset, ToolGen achieves improvements of 40.0% and 25.0% in Pass@1 for CodeT5 and CodeLlama, respectively.

==> src/evaluation.tex <==
\section{Evaluation}

We conduct extensive experiments to evaluate the effectiveness of \App in repository-level code generation. 

==> src/implementation.tex <==
\subsection{Approach Implementation}
Although \app is designed to be language-agnostic, our current focus is on developing a Python-specific prototype of \app.

\textbf{Base Model.}
In \app, we explore the utilization of three distinct code LLMs to encompass diverse model architectures and parameter scales:
\begin{itemize}
    \item \textbf{CodeGPT:} CodeGPT~\cite{CodeGPT} falls into the category of decoder-only models. It undergoes pre-training on a Python corpus sourced from the CodeSearchNet dataset~\cite{CodeSearchNet}, comprising 1.1 million Python functions. For our purposes, we adopt the pre-trained \emph{CodeGPT-small} version\footnote{https://huggingface.co/microsoft/CodeGPT-small-py}, which encompasses 124 million model parameters.

    \item \textbf{CodeT5:} CodeT5~\cite{CodeT5} belongs to the encoder-decoder model category and is similarly pre-trained on the Python corpus from the CodeSearchNet dataset. We select the pre-trained \emph{CodeT5-base} version\footnote{https://huggingface.co/Salesforce/codet5-base}, which comprises 220 million model parameters.

    \item \textbf{CodeLlama:} CodeLlama~\cite{CodeLlama} represents another decoder-only model, specialized for code-related tasks and based on Llama2~\cite{Llama2}. It is pre-trained on an even larger Python corpus, encompassing a staggering 100 billion tokens sourced from a Python-centric dataset~\cite{CodeLlama}. For our purposes, we adopt the pre-trained \emph{CodeLlama-7b} version\footnote{https://huggingface.co/codellama/CodeLlama-7b-Python-hf}, featuring a substantial 7 billion model parameters.
\end{itemize}
% Note that when feeding the code LLMs, we include the function signatures into the docstrings.



\textbf{Autocompletion Tool.}
We employ Jedi~\cite{Jedi} as our autocompletion tool. Jedi is a static analysis tool designed for Python, commonly utilized within integrated development environments (IDEs) and editor plugins. Utilizing Jedi, \app can trigger autocompletion, generating a list of suggestions that encompasses \emph{repository-level dependencies}, including user-defined attributes and functions.


\textbf{Code Augmentation.}
To create the augmented dataset for fine-tuning the employed base model, we begin with the Python corpus from the CodeSearchNet dataset. Since the CodeSearchNet dataset does not provide complete code repositories from which to extract Python functions, we initiate the process by crawling the code repositories listed in the dataset. Subsequently, we follow the procedure outlined in Section~\ref{sec:augmentation} to extract and augment functions within these code repositories, ultimately generating the augmented dataset.
It's important to note that the CodeSearchNet dataset includes a partitioning into training, validation, and test sets. For our code augmentation process, we exclusively utilize the code repositories associated with the training set. The resulting augmented dataset comprises a total of 256,870 pairs of docstrings and augmented functions, which are sourced from 12,231 distinct Python code repositories. Regarding dataset statistics, the average token count for docstrings is 10.96, and for augmented functions, it is 54.13. Additionally, the special token \comp appears an average of 5.37 times within these functions.

\textbf{Model Fine-tuning.}
In the fine-tuning process, we adopt different strategies for CodeGPT, CodeT5, and CodeLlama:
For CodeGPT and CodeT5, we perform full-parameter fine-tuning, optimizing all model parameters during this phase.
In the case of CodeLlama, we employ LoRA with a reduction factor (\emph{r}) of 16 and a scaling factor (\emph{alpha}) of 16 to achieve parameter-efficient fine-tuning. This approach allows us to optimize only 0.25\% of the trainable parameters in comparison to the original CodeLlama model.
The fine-tuning settings for learning rate and batch size are consistent across all three models, with a learning rate of 5E-6 and a batch size of 32. However, the number of epochs differs: 10 epochs for CodeGPT and CodeT5, while CodeLlama undergoes fine-tuning for 2 epochs. To ensure reproducibility, we set the seed for random functions to 42 consistently across all packages and libraries used.



\textbf{Tool-integrated Generation.}
\todo{details...}
